Learning Visual Composition through Improved Semantic Guidance

Visual imagery does not consist of solitary objects, but instead reflects the composition of a multitude of fluid concepts. While there have been great advances in visual representation learning, such advances have focused on building better representations for a small number of discrete objects bereft of an understanding of how these objects are interacting. One can observe this limitation in representations learned through captions or contrastive learning -- where the learned model treats an image essentially as a bag of words. Several works have attempted to address this limitation through the development of bespoke learned architectures to directly address the shortcomings in compositional learning. In this work, we focus on simple, and scalable approaches. In particular, we demonstrate that by substantially improving weakly labeled data, i.e. captions, we can vastly improve the performance of standard contrastive learning approaches. Previous CLIP models achieved near chance rate on challenging tasks probing compositional learning. However, our simple approach boosts performance of CLIP substantially and surpasses all bespoke architectures. Furthermore, we showcase our results on a relatively new captioning benchmark derived from DOCCI. We demonstrate through a series of ablations that a standard CLIP model trained with enhanced data may demonstrate impressive performance on image retrieval tasks.

==> sections/imagenet-table.tex <==
\begin{table*}[t]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{llcccccc}
\toprule
& & ImageNet \cite{deng2009imagenet} & ImageNet-A \cite{hendrycks2021nae} & ImageNet-R \cite{hendrycks2021many} & ImageNet-V2 \cite{recht2019imagenet} & ImageNet-Sketch \cite{wang2019learning} & ObjectNet \cite{2019objectnet} \\
\midrule
%\multicolumn{7}{c}{Prior Work} \\
CLIP \cite{pmlr-v139-radford21a} & & 76.2 & 77.2 & 88.9 & 70.1 & 60.2 & 72.3 \\
ALIGN \cite{pmlr-v139-jia21b} & & 76.4 & 75.8 & 92.2 & 70.1 & 64.8 & 72.2 \\
CoCa \cite{yu2022} & & 82.6 & 76.4 & 93.2 & 76.5 & 71.7 & 71.6 \\
\midrule
%\multicolumn{7}{c}{Our Method} \\
\multirow{5}{*}{{\bf Ours}} & {Ours (no JFT)} & 68.4 & \todo{27.2} & \todo{72.7} & \todo{62.8} & \todo{63.5} & \todo{?} \\
& {Ours (with JFT)} & 79.1 & 42.4 & 80.6 & 72.8 & 68.4 & \todo{?} \\
\bottomrule
\end{tabular}}
%\vspace{0.05cm}
\caption{{\bf Zero-shot image classification results}. Prior work performance derived from \cite{yu2022}. CoCa results report base model.\label{table:zero-shot}}
\end{table*}
